Examining Machine Learning for 5G and Beyond through an Adversarial Lens

Spurred by the recent advances in deep learning to harness rich information hidden in large volumes of data and to tackle problems that are hard to model/solve (e.g., resource allocation problems), there is currently tremendous excitement in the mobile networks domain around the transformative potential of data-driven AI/ML based network automation, control and analytics for 5G and beyond. In this article, we present a cautionary perspective on the use of AI/ML in the 5G context by highlighting the adversarial dimension spanning multiple types of ML (supervised/unsupervised/RL) and support this through three case studies. We also discuss approaches to mitigate this adversarial ML risk, offer guidelines for evaluating the robustness of ML models, and call attention to issues surrounding ML oriented research in 5G more generally.

==> 9authors.tex <==









\begin{IEEEbiographynophoto}{Rupendra Nath Mitra} is currently a doctoral student in the School of Informatics at The University of Edinburgh, UK. His research interest includes Wireless Networking, 5G security, and Machine Learning with applications to Cyber-Physical Systems. He received MS degrees in computer science and engineering from The Ohio State University and the University of Cincinnati, OH, USA. URL: http://www.rupenmitra.com/
\end{IEEEbiographynophoto}

\begin{IEEEbiographynophoto}{Mahesh K. Marina} is a Professor in the School of Informatics at the University of Edinburgh and a Turing Fellow at the Alan Turing Institute in London. Before joining Edinburgh in 2006, he had a two-year postdoctoral stint at the UCLA Computer Science Department. He received his PhD in Computer Science from the State University of New York at Stony Brook in 2004. He has previously held visiting researcher positions at ETH Zurich and at the Ofcom Headquarters in London. He is a Distinguished Member of the ACM and a Senior Member of the IEEE. More information about him and his research can be found at http://homepages.inf.ed.ac.uk/mmarina/.
\end{IEEEbiographynophoto}

\enlargethispage{-9cm}
